R&D for the CLIC Vertex and Tracking detectors

Significant progress has been made to develop silicon pixel technologies for use in the vertex and tracker regions of the proposed Compact Linear Collider (CLIC) detector design. The electron-positron collisions generated by this linear accelerator provide a clean, low-radiation environment for the inner detectors. However, physics-driven performance targets, the CLIC beam structure, and occupancies from beam-induced backgrounds place challenging requirements on detector technologies for this region. A pixel pitch down to 25 x 25$\mu$m$^{-2}$, material budget $\leq$ 0.2-2$\%X_0$ per layer, average power dissipation of down to 50mWcm$^{-2}$, position resolution of 3-7$\mu$m, and timing resolution as low as 5ns are called for in the vertex and tracking detectors. To this aim, a comprehensive R&D programme is ongoing to design and test silicon pixel detectors to fulfil these specifications, including both monolithic and hybrid devices. These studies involve Allpix$^2$ Monte Carlo and TCAD simulations, advanced 65nm ASIC and sensor design, laboratory testing, and beam tests of individual modules to determine the required performance parameters. The characterisation and simulation modelling of these devices has also lead to the development of a set of tools and software within the CLIC detector and physics (CLICdp) collaboration. This publication will present recent results from the technologies being developed and tested in view of the CLIC vertex and tracking detector requirements, such as various monolithic CMOS sensors, and fine pitch hybrid assemblies with planar sensors.

==> chapters/technologies.tex <==
\section{Pixel detector technologies}
\label{ch:technologies}
%%%%%%
\subsection{CLICpix2 with planar sensors}
CLICpix2, see Figures~\ref{fig:CPX2_photo} and~\ref{fig:CPX2_staggeredactiveedge}, is a small-pitch, pixelated readout chip designed to fulfil the needs of the vertex detector~\cite{cpx2_manual}.
It is part of the Timepix/Medipix family and is the successor to the CLICpix technology.
CLICpix2 ASICs have been solder bump-bonded to planar silicon sensors of thicknesses \SI{50}{\um} to \SI{200}{\um}~\cite{detector_tech_report}.

\begin{figure}[tb]
\centering
\begin{minipage}{.48\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figures/clicpix2_planar.png}
    \caption{Image of a CLICpix2 ASIC wire-bonded to a readout PCB (bottom)~\cite{detector_tech_report}.}
    \label{fig:CPX2_photo}
\end{minipage}%
\hfill
\begin{minipage}{.48\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figures/cpx2_staggerededge_croppedpng.png}
    \caption{Image of the CLICpix2 ASIC showing the staggered active edge design.}
    \label{fig:CPX2_staggeredactiveedge}
\end{minipage}  
\end{figure}

\textbf{Detector design :} The chip is designed in a $\SI{65}{\nm}$ CMOS process~\cite{detector_tech_report}.
Its pixel matrix consists of 128$\times$128 square pixels of pitch $\SI{25}{\um}$~\cite{cpx2_manual}.
A frame-based readout scheme is employed, where the in-pixel digital back-end can record three different measurements: ToT, ToA, and event counts.
These are combined into four CLICpix2 operational modes: simultaneous 8-bit ToA and 5-bit ToT, simultaneous 8-bit count and 5-bit ToT, 13-bit ToA, or 13-bit measurement of counts~\cite{cpx2_manual}. 

\textbf{Laboratory results :} A single-chip bump-bonding process is being developed at IZM~\cite{IZM} for CLICpix2 carrier wafers and active-edge sensors from FBK-CMM~\cite{FBK} and Advacam~\cite{Advacam}~\cite{detector_tech_report}.
Each of these devices were thoroughly tested in the laboratory using a combination of threshold equlisation, I-V scans, test pulses, and radioactive source exposures.

\textit{Test pulse measurements:} Charge of a known magnitude was directly injected into the CLICpix2 ASIC frontend so that the ASIC response per pixel could be seen independently from the sensor and bonding quality.
In the data analysis, pixels that recorded an event fewer than 10\% of the total number of pulses sent are said to be 'unresponsive'. 
This is either due to the pixel readout being masked due to high noise, being electrically connected to a large number of shorted pixels, or the pixel has a non-functioning frontend. 
Some pixels were found to record erroneous hits while other pixels were test pulsed, and if this occurs during $\geq$90\% of the test pulses of a neighbouring pixel then these are called 'unexpected' pixel responses.
This unwanted response can be caused by electrical connections between neighbouring pixels or noisy pixels.

All other pixels are split into two groups with respect to the average number of counts recorded during test pulsing.
Due to the charge injection method, it is expected that the signal crosses the pixel threshold twice for each pulse injection.
Therefore pixels with an average number of counts between 2 and 1.5 inclusively as expected are said named 'double crossing'.
Other pixels are said to be 'single crossing' and likely have a weak frontend response.

\textit{Radioactive source exposure:} To investigate the behaviour of each CLICpix2 assembly to ionising particles, a Sr-90 radioactive source was placed above the assembly to obtain evenly distributed hits across the pixel matrix. 
A histogram of the pixel hit rates is then fitted by a Gaussian function, and the expected pixel behaviour is for the total number of hits for a pixel to be within 3$\sigma$ of the Gaussian mean.
The tails above and below the 3$\sigma$ cut correspond to pixels that are deemed to be 'high rate' or 'low rate' respectively.
The Gaussian peak contains 99.7\% of all pixels, therefore in a perfect assembly 25 pixels are expected to be high rate and 25 to be low rate.  

\textit{Pixel categorisation:} To better understand the assembly performance, the results from the described laboratory measurements are combined to classify pixels into seven categories. 
These data-driven category definitions are detailed below.
It is noted that each pixel can only be in one category, with preceding categories taking precedence. 
\begin{enumerate}
    \item Masked: Pixels of this category have been masked during threshold equalisation or by the user due to large noise. No information is gathered from these pixels, therefore their response cannot be characterised.
    \item Unresponsive: Pixels in this category responded less than 10\% of the time to charge injection.
    \item Shorted: The pixel records unexpected hits when not pulsed $\geq$90\% of the time. 
    \item Bonding or sensor issues: Pixels in this set were found to be double crossing and low rate, so are said to have bonding or sensor issues. 
    \item Single crossing: These pixels were found to be single crossing during test pulsing measurements.
    \item High rate: This set of pixels were found to have a high rate during a source measurement. 
    %These pixels arise from edge effects due to the active-edge present. ->> ask Dominik D. about this
    \item Expected response: The expected responses are seen in all tests for this pixel: double crossing test pulse response, normal rate from source measurement, no other issues.
\end{enumerate}
The categorisation results for assembly 20 are presented in Table~\ref{tab:cpx2_categories} and Figure~\ref{fig:cpx2_categories}.
The majority of high rate pixels for this device are located 1-2 rows/columns from the matrix edge. 
One possible explanation for this effect is that the electric field distribution from the staggered active edge design, see Figure~\ref{fig:CPX2_staggeredactiveedge}, causes rows/columns 1-2 to receive a lower amount of charge, while rows/columns 2-3 receive a higher amount.
Using the categorisation results, an interconnect yeild of $15757/(128\times128 -32 -2) = 96.4\%$ was calculated.
This is the highest interconnect yeild obtained for a CLICpix2 planar assembly so far.
The yield of high-quality assemblies is low due to the challenging bump-bonding process for the small pitch size. 
It was found that the combination of Ti/W/Cu Under Bump Metalisation (UBM) used by FBK-CMM and SnAg bump material used by IZM produced the best results.

\begin{table}[tb]
  \begin{minipage}[c]{0.4\textwidth}
    \caption{Summary of categorisation results of CLICpix2 assembly 20.}
    \label{tab:cpx2_categories}
    \centering
    \begin{tabular}{ll}
      \toprule
      \multirow{2}{*}{\textbf{Category}}  & \textbf{Number}\\
                                          & \textbf{of Pixels}              \\
    \midrule	
	  1. Masked			& 32\\
    \midrule
	  2. Unresponsive		& 2\\
      \midrule
	  3. Shorted			& 2\\
    \midrule
	  4. Bonding or			& \multirow{2}{*}{344}\\
	     sensor issues			&		\\
    \midrule
	  5. Single crossing		& 0\\
    \midrule
	  6. High rate		   	& 247\\
    \midrule
	  7. Expected response		& 15757\\
    \bottomrule
    \end{tabular}
  \end{minipage}\hfill
  \begin{minipage}[c]{0.55\textwidth} 
    \centering
    \includegraphics[width=\linewidth]{figures/categories_as20_clicdp.png}
    \caption{A 2D map showing the categories determined for each pixel of CLICpix2 planar assembly 20.}
    \label{fig:cpx2_categories}
  \end{minipage}
\end{table}


\textbf{Test-beam results :} Assembly 20 was tested using the DATURA beam telescope set-up~\cite{EUDET_telescope_paper} in the DESY II test-beam area~\cite{DESYpaper}.
The DESY-II synchrotron supplies an electron-positron particle beam of energies up to \SI{6}{GeV}, and a nominal beam energy of \SI{5.4}{GeV} was chosen for data taking to increase the gained statistics.
For the set-up used, the telescope resolution at the DUT plane was calculated to be \SI{2.5}{\um}.
The nominal operating conditions for CLICpix2 assembly 20 were determined during the laboratory testing: a threshold of approximately \SI{645}{electrons} and a bias voltage of \SI{-60}{V}.

%%results from DESY for as20: voltage scan, threshold scan
By varying the bias voltage applied, the optimal applied bias voltage and depletion voltage can be determined.
Figure~\ref{fig:cpx2_voltagescan_clusterplots} presents such a scan for assembly 20 with two observable quantities: the mean size of track-associated clusters and the Most Probable Value (MPV) from a Landau-Gaussian fit to the associated cluster charge distribution.
Examining the first data set, it is seen that the bias voltage that produces the highest mean cluster size in this scan, and therefore the maximum amount of charge sharing, is \SI{-25}{V}.
This is therefore the optimal operational bias voltage for this device.
To calculate the depletion voltage of the assembly, two first order polynomial functions were fit to the linear ranges of the histogram of MPV$^2$ vs bias voltage.
The $X$ coordinate of the intersection point for these two functions provides the depletion voltage, which was calculated to be \SI{-24}{V} for this sample.

\begin{figure}[tb]
 \begin{minipage}[t]{0.48\textwidth} 
 \centering
    \includegraphics[width=\linewidth]{figures/clicpix2_voltagescan_overlay.png}
    \caption{Histogram of test-beam data for CLICpix2 planar assembly 20, showing mean track-associated cluster size vs applied bias voltage, and MPV of a Landau-Gaussian fit to the track-associated cluster charge vs applied bias voltage.}
    \label{fig:cpx2_voltagescan_clusterplots}
 \end{minipage}\hfill
 \begin{minipage}[t]{0.48\textwidth} 
 \centering
    \includegraphics[width=1.05\linewidth]{figures/comparison_efficiency_as20_desyjuly_-25_-60.pdf}
    \caption{Comparison of the effiency curves obtained from threshold scans of assembly 20 a bias voltages of \SI{-25}{V} and \SI{-60}{V}.}
    \label{fig:cpx2_thresholdscan_eff}
 \end{minipage}
\end{figure}

Test-beam analysis has calculated the efficiency of this assembly to be 98.1\% at nominal conditions, though higher efficiencies have been measured for similar samples using data from the SPS test-beam facility~\cite{}.
The device detection threshold was scanned from \SI{0.5}{kelectrons} to \SI{15.9}{kelectrons}, and the resultant trends are shown in Figure~\ref{fig:cpx2_thresholdscan_eff}.
The efficiency curve for two values of bias voltage, \SI{-25}{V} and \SI{-60}{V}, are shown where the efficiency falls with increaing threshold as expected.
Both data curves plateau at 98.1\% for thresholds up to \SI{2.0}{kelectrons}, then effiencies begin to decrease until a minimum value at \SI{15.9}{kelectrons} of 13.5\% and 8.9\% for \SI{-60}{V} and \SI{-25}{V} respectively.

%%%%%%

\subsection{ELADs}
The positional resolution of thin sensors is limited to $pitch/\sqrt{12}$ due to the limited charge sharing when traversing the small sensor thickness.
Reducing the pixel size can improve this, however the pitch is often limited by the feature sizes of the readout electronics.
The Enhanced LAteral Drift (ELAD) design enhaces the lateral drift in the sensor layer to increase charge sharing between adjacent pixels.
ELAD sensors allow the positional resolution to be improved without the need to adapt the pixel pitch and/or sensor thickness~\cite{detector_tech_report}.
This technology is targetting the requirements of the CLICdet vertex detector.
Due to the multiple layers needed of ion implantation and epitaxial growth, the manufacture of ELADs is challenging.
The first set of ELAD assemblies are in production to demonstrate the performance capabilities of this concept.

\textbf{Simulation results :} Deep ion implants inside the sensor are used to adapt the electric field to both promote lateral drift and reduce low electric field regions~\cite{detector_tech_report}. 
The postition, dimensions, number, and doping concentrations of the implants were simulated using a 2D TCAD finite element simualtions~\cite{synopsys-tcad} to optimise the sensor design.
In Figure~\ref{fig:elad_tcad} the implant design developed from these investigations can be seen in a TCAD transient simualtion.
The electron current density is plotted after a minimally ionising particle hit the sensor surface at a distance of \SI{16.9}{\um} from the left-hand pixel implant.

\begin{figure}[tb]
\begin{minipage}[t]{0.24\textwidth} 
    \centering
    \includegraphics[width=0.94\linewidth]{figures/elad_transient_cropped.png}
    \caption{TCAD simulation of an ELAD sensor after an incident MIP~\cite{detector_tech_report}.}
    \label{fig:elad_tcad}
 \end{minipage}\hfill
 \begin{minipage}[t]{0.72\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figures/small_elad_simulation.png}
    \caption{\apsq simulation of the charge collected by adjacent strips in a ELAD detector vs. distance.
    A position of \SI{0}{\um} corresponds to the center of the first strip, and \SI{27.5}{\um} to the center between the two strips.}
    \label{fig:elad_resolution}
 \end{minipage}
\end{figure}

The detector performance parameters were investigated through \apsq simulations.
For a pixel pitch of \SI{55}{\um}, the ELAD detector has a factor of two improvement from the binary positional resolution comapred to a standard planar sensor.
In another \apsq simulation study, the collected charge between two strips in an ELAD detector was modelled as a function of MIP incidence position.
As seen in Figure~\ref{fig:elad_resolution}, the theoretical optimum is a linear charge sharing between the two strips, with maximal sharing when the particle is incident at the center between both strips.
The ELAD simulations are much closer to this calculated optimum than the standard case, thus it can improve upon the binary limit of $strip\_distance/\sqrt{12}$.

%%%%%%
\subsection{CLICTD}
The monolithic CLIC Tracking Detector (CLICTD) targets the requirements of the tracking detector.
It is produced using a \SI{180}{\nm} modified HRCMOS imaging process~\cite{clictd_proceedings}.

\textbf{Detector design :} CLICTD features a 128$\times$16 matrix with pixels of pitch \SI{300}{\um}$\times$\SI{30}{\um}~\cite{detector_tech_report}.
Each pixel is further segmented into eight subpixels of size \SI{37.5}{\um}$\times$\SI{30}{\um} to decrease the charge collection time while mainting a low amount of digital circuitry per pixel.
Three pixel data modes are implemented: simultaneous 8-bit integrated Time-over-Threshold (ToT) and 5-bit Time-of-Arrival (ToA) of the first hit subpixel; 13-bit ToA of the first hit subpixel; and event counts of each subpixel.
The data readout uses a rolling shutter scheme as the pixel occupancies in the CLIC tracking detector are estimated to be near one hit per bunch crossing.

Figure~\ref{fig:clictd_1} presents the design of two pixels in CLICTD.
Charge is collected by a small collection electrode situated inside a low-dose N-type implant, itself placed above a P-type expitaxial layer~\cite{clictd_proceedings}.
To ensure full lateral depletion, low dose deep N-implants and a HR epitaxial layer are used~\cite{detector_tech_report}.
A modified design has introduced a gap in the N layer to reduce the charge collection time further, this design is shown in Figure~\ref{fig:clictd_2}.
CLICTD aims to have a small capacitance in the order of fF; low detection threshold of approximately \SI{180}{electrons}; low power consumption; and a large signal-to-noise ratio.

\begin{figure}[tb]
\centering
\begin{minipage}{.48\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figures/clipped_process_2.png}
    \caption{Diagram of the CLICTD detector with a continous N layer design~\cite{clictd_proceedings}.}
    \label{fig:clictd_1}
\end{minipage}%
\hfill
\begin{minipage}{.48\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figures/clipped_process_1.png}
    \caption{Diagram of the CLICTD detector with an additional N layer gap design~\cite{clictd_proceedings}.~}
    \label{fig:clictd_2}
\end{minipage}  
\end{figure}

\textbf{Simulation results :} Due to the complex, non-linear nature of the electric field in this device, the design of CLICTD was optimised through detailed TCAD simualtions~\cite{detector_tech_report}.
Currently, MC simualtions using \apsq are being carried out to better understand the response of the samples in labortory and test beam measurements.

\textbf{Laboratory results :} CLICTD samples have been produced using both design layouts.
The I-V characteristics of these assemblies was measured for multiple P well bias voltages.
It was found that the substrate in the continuous deep N-type implant design can be biased to higher magnitudes due to it having a better isolation between the substrate and the P wells~\cite{clictd_proceedings}.
After equalisation of the pixel matrix, a threshold dispersion of approximately \SI{16}{electrons} was extracted for sample B1, see Figure~\ref{fig:clictd_equalisation}.
This assembly was produced with the additional N layer gap design and was operated at a p-well/substrate bias voltage of -3/\SI{-3}{\V}.
CLICTD chips have been exposed to X-rays produced from multiple target materials to determine the \SI{16}{electrons} per DAC conversion factor between threshold DAC value and the threshold level in electrons~\cite{clictd_proceedings}.
The ToT response of a single pixel of CLICTD sample A1 is presented in Figure~\ref{fig:clictd_tot}.
Assembly A1 has the continuous N layer design and was operated at a threshold of approximately \SI{330}{electrons} and a p-well/substrate bias voltage of -3/\SI{-6}{\V}.

\begin{figure}[tb]
\centering
\begin{minipage}{.48\textwidth}
    %\centering
    \includegraphics[width=1.05\linewidth]{figures/equalised_clictd_sample_b1.png}
    \caption{Equalisation histograms for CLICTD sample B1.
    Data was taken at maximum and minimum local threshold settings to determine the equalised value of the threshold adjustment for each pixel.}
    \label{fig:clictd_equalisation}
\end{minipage}%
\hfill
\begin{minipage}{.48\textwidth}
    %\centering
    \includegraphics[width=1.05\linewidth]{figures/clictd_totspectrum.png}
    \caption{Scan of ToT value of pixel 0,0 of CLICTD sample A1.
    Test pulses of different magnitudes were used to inject charge into the pixel, and the ToT value obtained was recorded.}
    \label{fig:clictd_tot}
\end{minipage}  
\end{figure}

%%%%%%
\subsection{ATLASPix}
Several monolithic HV-CMOS sensors have been developed for the upgrade of the ATLAS pixel detector outer layer.
The ATLASpix\_Simple is interesting to CLIC as it targets similar requirements to the those of the CLIC tracking detector.
Assemblies with resistivities from \SI{20}{\ohm\cm} to \SI{1000}{\ohm\cm}, and total thicknesses of \SI{62}{\um} and \SI{100}{\um}, have been produced and studied.

\textbf{Detector design :} This HV monolithic active pixel sensors (HV-MAPS) was produced using a commerical \SI{180}{\nm} HV-CMOS processing method.
Elongated pixels of pitch \SI{130}{\um}$\times$\SI{40}{\um} are arranged in a matrix of 25 columns and 400 rows.
ATLASpix\_Simple has a fully integrated readout, fast charge collection using drift, and a low material budget.
Each pixel is capable of recording a 10-bit ToA and a 6-bit ToT.

\textbf{Test-beam results :} Samples of three different resistivities and two different thicknesses were tested at the DESY test-beam facility~\cite{DESYpaper} to evalue their performance.
Each device was nomially operated at a bias voltage of \SI{-50}{\V} and a threshold of approximately \SI{650}{electrons}.
The data curves in Figure~\ref{fig:atlaspix_eff} show the distributions of efficiency vs. threshold level for three samples.
Efficiencies of 98-99\% were achieved for the nominal operational conditions, though higher efficiencies have been measured for similar samples using data from the SPS test-beam facility.
Compared to the other resistivities, the \SI{20}{\ohm\centi\meter} assembly has a larger plataeu region before the efficiency decreases for higher threholds, eventually dropping to be near 0\% .

The time residuals between the track and cluster timestamps for the same three samples are shown in Figure~\ref{fig:atlaspix_timing}.
It is seen that the \SI{20}{\ohm\centi\meter} detector has a slower timing response and is subject to a larger timewalk effect when compared to the other two detectors.

\begin{figure}[tb]
\begin{minipage}[t]{0.48\textwidth} 
    \centering
    \includegraphics[width=\linewidth]{figures/atlaspix_efficiency.png}
    \caption{Efficiency as a function of threshold for three ATLASPix\_Simple detectors.}
    \label{fig:atlaspix_eff}
 \end{minipage}\hfill
 \begin{minipage}[t]{0.48\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figures/atlaspix_timing.png}
    \caption{Time residual distributions for three ATLASPix\_Simple detectors.}
    \label{fig:atlaspix_timing}
 \end{minipage}
\end{figure}








